Time-Efficient Qudit Gates through Incremental Pulse Re-seeding

Current efforts to build quantum computers focus mainly on the two-state qubit, which often involves suppressing readily-available higher states. In this work, we break this abstraction and synthesize short-duration control pulses for gates on generalized d-state qudits. We present Incremental Pulse Re-seeding, a practical scheme to guide optimal control software to the lowest-duration pulse by iteratively seeding the optimizer with previous results. We find a near-linear relationship between Hilbert space dimension and gate duration through explicit pulse optimization for one- and two-qudit gates on transmons. Our results suggest that qudit operations are much more efficient than previously expected in the practical regime of interest and have the potential to significantly increase the computational power of current hardware.

==> abstract.tex <==
\begin{abstract}
Current efforts to build quantum computers focus on the realization of noise-robust two-level systems, so called qubits, that can be manipulated by applying quantum gates. However, in many proposed architectures a greater number of energy levels are accessible and a physical qubit is achieved by selecting two of them. While this artificial abstraction allows a direct correspondence to classical logic, operating on a larger Hilbert space readily available is promising. On a hardware level, quantum gates are implemented via analog pulses, and being able to realize high-fidelity pulses directly impacts the quality of a quantum processor. In this work we focus on synthesizing short-duration pulses for higher dimensional qudits by employing quantum optimal control methods. To this end we use the open-source software packages Juqbox and Quandary. We specifically look at single-qudit and two-qudit operations and investigate the pulse time scaling with respect to the qudit dimension. Since the success of optimal control algorithms usually depends on the initial guess of a pulse, we furthermore present an efficient procedure to seed the optimizer.
\end{abstract}
